Interaction Region Visual Transformer for Egocentric Action Anticipation

Human-object interaction is one of the most important visual cues and we propose a novel way to represent human-object interactions for egocentric action anticipation. We propose a novel transformer variant to model interactions by computing the change in the appearance of objects and human hands due to the execution of the actions and use those changes to refine the video representation. Specifically, we model interactions between hands and objects using Spatial Cross-Attention (SCA) and further infuse contextual information using Trajectory Cross-Attention to obtain environment-refined interaction tokens. Using these tokens, we construct an interaction-centric video representation for action anticipation. We term our model InAViT which achieves state-of-the-art action anticipation performance on large-scale egocentric datasets EPICKTICHENS100 (EK100) and EGTEA Gaze+. InAViT outperforms other visual transformer-based methods including object-centric video representation. On the EK100 evaluation server, InAViT is the top-performing method on the public leaderboard (at the time of submission) where it outperforms the second-best model by 3.3% on mean-top5 recall.

==> intro.tex <==
%\textbf{Interactions model attends to objects that are important for the current action and will be used in the next action.}

Egocentric action anticipation is crucial for developing AI assistants for surgery~\cite{sexton2018anticipation},  assembly~\cite{chen2018software}, and construction~\cite{sherafat2020automated}.
Egocentric action anticipation is also becoming a viable technology thanks to wide use of wearable cameras such as GoPro~\cite{Liu_2022_CVPR}.
In egocentric action anticipation, the model predicts the immediate action that is going to happen, usually 1 second into the future~\cite{furnari2020rolling}.
However, the observed video may not contain sufficient visual cues and semantics to predict the future actions accurately.
Therefore, it is important to leverage all available information when predicting future actions.
%One of the biggest challenges in egocentric  action anticipation is determining which object(s) will be used.
It is well known that relationships between objects and humans indicate the actions humans are executing. 
A recent line of work explored these properties for effective action recognition~\cite{ou2022object} and action anticipation~\cite{roy2021action}. 
We propose to exploit the contextual visual changes in humans and objects during an interaction to boost  anticipation.
This type of visual information is significant for action anticipation.
For example, when standing in front of the sink, \textit{putting down a used pan} or \textit{opening the tap} are probable future actions.  
In this instance, the likely future action depends on whether the observed interaction is \textit{serving food from a pan} or \textit{picking up a glass} as shown in \cref{fig:motivation}. 
%However, the observed action label is not available for egocentric action anticipation.
Therefore, we propose to model the interactions between hands and objects using a novel visual transformer model where the attention weights determine informative interactions for predicting the next action.

More specifically, the human hands contribute more to the visual change of the interacting object(s) in egocentric videos~\cite{dessalene2020egocentric, cheng2022team}.
Similarly, the appearance of the hand is affected mostly by the interacting objects.
For example, a spoon's appearance is different when it is used for feeding compared to when it lies on a table.
Our hand also looks different when it holds a spoon compared to a plate.
Another motivation to model all the hand-object interactions is some actions are better represented by more than one interaction. 
In such a case, we need to consider other objects around the hand apart from the object involved in the next action.
For example, a knife is crucial to \textit{cut} a \textit{pizza}.
So, both \textit{holding} knife and \textit{pizza} are essential for anticipating \textit{cut pizza}.



\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/motivation-3.pdf}
    \caption{Modeling hand-object interactions and infusing environment to predict the next action. We model the interactions between the hand and the pan while serving food. We infuse the environment context containing the empty pan into the interactions to predict the next action.}
    \label{fig:motivation}
\end{figure}

% In Figure \cref{fig:motivation}(b), we show that interaction modeling attends to the \textit{knife}, \textit{pizza} and where the left \textit{hand} holds the pizza to correctly anticipate \textit{cut pizza}.
% We accurately predict next actions based on modeling interactions with multiple active objects.

%\textbf{Interaction modeling in anticipation.}
Although hand-object interactions are critical for action anticipation, most prior works only focus on the appearance of the entire video~\cite{girdhar2021anticipative,wu2022memvit}, motion~\cite{rodriguez2018action}, detected objects~\cite{furnari2020rolling}, or a combination of all of the above~\cite{furnari2020rolling,sener2020temporal}.
Although \cite{roy2021action} presents a model for human-object interactions for action anticipation, it does not exploit the visual changes in humans and objects' appearance caused by the execution of actions.
\emph{We propose a novel way to model human-object interactions that involve computing the change in the appearance of objects and humans due to executing the action.}
In fact, specific actions may cause specific changes in the appearance of objects, the environment, and even the appearance of hands.
We design a spatio-temporal visual transformer denoted as human-object Interaction visual transformer (InAViT) for action anticipation that refines \emph{interaction tokens} in every frame. 
The interaction tokens are obtained from refined object and human tokens and the refinement is influenced by objects, hands, and the anticipated action.
We incorporate the environment information (contextual cues) into interaction tokens by proposing a trajectory cross-attention mechanism based on trajectory attention~\cite{patrick2021keeping}.
Finally, we infuse interaction tokens into the observed video to build an interaction-centric video representation for effective action anticipation.

Human-object interactions in actions are expressed as relations in spatio-temporal graphs~\cite{jain2016structural, wang2018videos, materzynska2020something, teng2021target, ou2022object}.
Our approach is inspired by these interaction representation-based approaches especially the progression of human-object relationships for action recognition tasks~\cite{ou2022object}.
However, our interaction-centric video representation recognizes humans as a separate entity from objects that affect visual change on objects and vice-versa.
Object-centric approaches consider only object dynamics ~\cite{herzig2022object, zhang2022object} and do not treat human hands as a separate entity~\cite{materzynska2020something}. 
However, consecutive egocentric actions may only be connected by hand movement.
For example, \textit{washing a dish} followed by \textit{closing tap} are connected only through hand movement. 
The hand causes a visual change in both these objects and also changes in appearance while interacting with them. 
Modeling the changes in both hand and objects through hand-object interactions connects these actions better than observing the change in objects alone. 
Therefore, we postulate that human-object interaction-centric representations are better suited for action anticipation than object-centric approaches.
Specifically, we leverage the recent trajectory attention-based MotionFormer model ~\cite{patrick2021keeping} to build the interaction-centric video representation. 
%Ideally, a model that represents interactions should cover both human-object and environment-human-object relationships.
%So, we model and refine interaction tokens in two steps.
%First, we propose spatial cross-attention between objects and hand representation to capture the visual change at every frame across hands and objects.
%Second, we propose trajectory cross-attention to refine the interaction tokens obtained in every frame in the first step using the environment.
%In spatial cross-attention, we refine hand and object tokens in each frame to obtain interaction tokens. 
%We pool the information across the object tokens in the frame as keys and values. 
%We refine the query hand token using those keys and values.
%Similarly, we refine each object token by pooling the information across other objects and hands. 
%We propose trajectory cross-attention to evaluate possible trajectories of the interaction tokens given the environment.
%We then pool the environment information first spatially and then temporally to refine the interaction tokens across the trajectory. 
In summary, our contributions are:
\begin{itemize}
    \item We propose a novel Transformer-based interaction model that computes appearance change in objects and hands occurring due to execution of action and models these changes in appearances to refine the video representation for action anticipation.
    To the best of our knowledge, we are the first to demonstrate the efficacy of hand-object interactions for egocentric action anticipation.
    \item On the EK100 evaluation server, our model InAViT is top the public leaderboard and outperforms the second-best model by 3.3\% on mean-top5 recall.
\end{itemize}
